Causal Linearizability: Compositionality for Partially Ordered Executions

In the interleaving model of concurrency, where events are totally ordered, linearizability is compositional: the composition of two linearizable objects is guaranteed to be linearizable. However, linearizability is not compositional when events are only partially ordered, as in many weak-memory models that describe multicore memory systems. In this paper, we present causal linearizability, a correctness condition for concurrent objects implemented in weak-memory models. We abstract from the details of specific memory models by defining our condition using Lamport's execution structures. We apply our condition to the C11 memory model, providing a correctness condition for C11 objects. We develop a proof method for verifying objects implemented in C11 and related models. Our method is an adaptation of simulation-based methods, but in contrast to other such methods, it does not require that the implementation totally order its events. We also show that causal linearizability reduces to linearizability in the totally ordered case.

==> refinement.tex <==
\section{Stepwise Refinement}

Correctness of an implementation structure can be judged by showing
\emph{refinement} against an abstract specification. In this section,
we develop a notion of refinement between execution structures.  Armed
with this notion of refinement, we can emulate well-established
methods for sequentially consistent architectures, and verify
correctness of an implementation via stepwise refinement of the traces
of a concurrent specification. % These are canonical objects in the case
% of linearizable data structures.

% and specifications such as TMS2 in the case of
% transactional memory \cite{}.

% There are several possible ways in which one could define refinement
% between execution structures.  One option is simply to define
% refinement as trace inclusion: so $C$ refines $A$ if all traces of
% $C$ are also traces of $A$. However, such a definition is
% unnecessarily strong.
Our notion of refinement between execution structures is given as
follows. Each refinement may ignore the real-time order between
operations (increase concurrency), but must preserve all the
communication required by the abstract execution structure.
\begin{definition}[Execution structure refinement]
\label{def:exec-ref}
An execution structure $\calE_B = (E_B, \HardArrow_B, \SoftArrow_B)$
{\em refines} an execution structure
$\calE_A = (E_A, \HardArrow_A, \SoftArrow_A)$, denoted
$\calE_B \leq \calE_A$ if (1) $E_B = E_A$; (2)
$\HardArrow_B \subseteq \HardArrow_A$; and (3)
$\SoftArrow_A \subseteq \SoftArrow_B$.
\end{definition}
% \fbox{is $E_B \subseteq E_A$ enough?}

This notion of refinement is sufficient is sound with respect to
causal linearizability, i.e., any refinement of a causally atomic
execution is itself causally atomic. This property is captured by
\refthm{thm:ref-causal-atom} below, which is the main result for this
section.
\begin{theorem}[Causal linearizability
  preservation]\label{thm:ref-causal-atom}
  If $\calE_A$ is a causally atomic execution structure (w.r.t. some
  sequential object), and $\calE_B \leq \calE_A$, then $\calE_B$ is also
  causally atomic (w.r.t the same sequential object).
\end{theorem}
% \begin{proof}
%   Because $\calE_A$ is causally atomic, there is some legal $k$
%   witnessing this fact. Thus $k$ also
%   witnesses the causal linearizability of $\calE_B$. \qed
% \end{proof}

\begin{corollary}\label{cor:ref-causal-opacity}
  For execution structures $\calE_A$ and $\calE_B$ such that
  $\calE_B \leq \calE_A$, if $\calE_A$ is causally linearizable, then
  so is $\calE_B$.
\end{corollary}

\fbox{Needs some text..}

The notion of refinement defined in \refdef{def:exec-ref} provides
sufficient conditions to ensure refinement of their abstractions for
any abstraction mapping.
\begin{lemma}\label{lem:lamp-atom-ref}
  Suppose $\calE_A = (E, \HardArrow_A, \SoftArrow_A)$ and
  $\calE_B = (E, \HardArrow_B, \SoftArrow_B)$ are execution structures
  and $\mu : E \to X$ is an execution mapping. If
  $\calE_B \leq \calE_A$ then
  $F_{\mu}(\calE_B) \leq F_{\mu}(\calE_A)$.
\end{lemma}
% \begin{proof}
%   The first property of \refdef{def:exec-ref} is immediate: both event
%   structures have event set $X$.  The second property of Definition
%   \ref{def:exec-ref} follows easily from the fact that
%   $\HardArrow_B \subseteq \HardArrow_A$.  Likewise, the third property
%   follows from the fact that $\SoftArrow_A \subseteq \SoftArrow_B$.
% \end{proof}


% \begin{proof}
%   By \reflem{lem:lamp-atom-ref}, we have
%   $F_{\gamma}(\calE_B) \leq F_{\gamma}(\calE_A)$, so the result follows from
%   \refthm{lem:ref-causal-atom} and the definition of causal opacity.
% \end{proof}


% We rely on the following lemma, which provides a sufficient condition
% on two causal histories to ensure refinement between the resulting
% execution structures.
% \begin{lemma}[Causal history refinement]
% \label{lem:ref-hist}
% If any two causal histories $h_B, h_A$ satisify $InvRes(h_A) \subseteq InvRes(h_B)$
% and $RespInv(h_B) \subseteq RespInv(h_A)$ then $\calE(h_A) \leq \calE(h_B)$ where
% \begin{align*}
% InvRes(h) = \{(i, r) \in h \mid i \in \Inv \wedge r \in Resp\} \\
% RespInv(h) = \{(r, i) \in h \mid i \in \Inv \wedge r \in Resp\}
% \end{align*}
% \end{lemma}
% \begin{proof}
% Immediate by construction.
% \end{proof}

% \newcommand{\IR}{{\it IR}}


% We rely on the following lemma, which provides a sufficient condition
% on two causal histories to ensure refinement between the resulting
% execution structures.
% \begin{lemma}[Causal history refinement]
% \label{lem:ref-hist}
% Suppose $\IR = \Inv \times \Resp$ and $RI = \Resp \times \Inv$. If
% $\causalord{\bbC}$ and $\causalord{\bbD}$ are causal histories of
% configurations $\bbC$ and $\bbD$ that satisify
% $(\mathord\causalord{\bbC} \cap \IR) \subseteq
% (\mathord\causalord{\bbD} \cap \IR)$ and
% $(\mathord\causalord{\bbC} \cap RI) \subseteq
% (\mathord\causalord{\bbD} \cap RI)$ then $\ES_\bbC \leq \ES_\bbD$.
% \end{lemma}
% \begin{proof}
% Immediate by construction.
% \end{proof}





%%% Local Variables:
%%% mode: latex
%%% TeX-master: "main.tex"
%%% End:

